Conditional Variational Capsule Network for Open Set Recognition

In open set recognition, a classifier has to detect unknown classes that are not known at training time. In order to recognize new categories, the classifier has to project the input samples of known classes in very compact and separated regions of the features space for discriminating samples of unknown classes. Recently proposed Capsule Networks have shown to outperform alternatives in many fields, particularly in image recognition, however they have not been fully applied yet to open-set recognition. In capsule networks, scalar neurons are replaced by capsule vectors or matrices, whose entries represent different properties of objects. In our proposal, during training, capsules features of the same known class are encouraged to match a pre-defined gaussian, one for each class. To this end, we use the variational autoencoder framework, with a set of gaussian priors as the approximation for the posterior distribution. In this way, we are able to control the compactness of the features of the same class around the center of the gaussians, thus controlling the ability of the classifier in detecting samples from unknown classes. We conducted several experiments and ablation of our model, obtaining state of the art results on different datasets in the open set recognition and unknown detection tasks.

==> sections/s0_abstract.tex <==
\begin{abstract}
In open-set recognition, a classifier has to detect unknown classes that are not seen during training, whereas standard classifiers support only known classes at test time. In order to recognize new classes the classifier has to project the input samples of known classes in very compact and separated regions of the features space in order to discriminate outlier samples of unknown classes. Recently proposed Capsule Networks have shown to outperform alternatives in many fields, particularly in image recognition, however they have not been fully applied yet to open-set recognition. In capsule networks, scalar neurons are replaced by capsule vectors or matrices, whose entries represent different properties of objects. In our proposal, during training, capsules features of the same known class are encouraged to match a pre-defined gaussian, one for each class. To this end, we use the variational autoencoder framework, with a set of gaussian prior as the approximation for the posterior distribution. In this way, we are able to control the compactness of the features of the same class around the center of the gaussians, thus controlling the ability of the classifier in detecting samples from unknown classes. We obtain competitive results with respect to previous works, outperforming state of the art methods by a large margin (from +9.95\% to +12.1\% of F1 score) on MNIST open-set classification.
\end{abstract}

==> sections/s1_introduction.tex <==
\section{Introduction}


\begin{figure}[ht]
    \centering
    \includegraphics[width=0.5\textwidth]{./plots/first_image_v8.png} \\
    \caption{VAECapOSR Model. Input samples are fed into the Capsule Network that produces distributions over the latent space. Each class has its own prior gaussian distribution in the feature space, that in the figure are represented as spheres. After training, the known samples (represented as small points) are clustered around the class target gaussians. The samples belonging to unknown classes are represented as black triangles, far from the target distributions.\label{fig:VAECapOSR}}
\end{figure}


Over the past decade, Deep Learning has become the dominant approach in Machine Learning,  achieving spectacular results on many visual recognition tasks \cite{imagenet, vgg16, resnet}. Notably, some recent developed models approach  human-level performance \cite{relu, deepface, conv}. However, almost all of them are proposed for closed set scenarios, where a critical assumption is that all samples should belong to at least one labeled category. When observing a sample from an unknown category, closed-set systems are forced to choose a class label for it from one of the known categories, which limits their usability in dynamic and ever-changing real applications.

To overcome such a limitation, the concept of open set recognition was proposed to enable the classification system to identify all of known categories, while simultaneously detecting unknown test samples. In the open set problem setting, samples included/excluded in label space are referred to as knowns/unknowns. Openset classifiers need to use incomplete knowledge learned from a finite set of accessible categories to devise effective representations separating knowns from unknowns. Early works have identified this issue, and have proposed methods employing forms of thresholding for rejection of unknowns \cite{tosr, towr}. Deep neural networks, despite demonstrating powerful capability in learning discriminative representations in closed environments, encounter accuracy degradation within open set settings \cite{topn}. As a naive strategy, modeling a threshold for SoftMax output has been demonstrated to be a sub-optimal solution for deep neural networks to identify unknowns. Thus the Extreme Value Theory was introduced to better adapt these discriminative models, fully based on supervised learning, for open-set settings. The underpinning idea is to calibrate SoftMax scores so to estimate the probability of unknowns \cite{crosr,topn}. In addition to deep discriminative models, deep generative models focusing on learning efficient latent feature representations by unsupervised leaning, have been widely utilized in open-set recognition tasks, and have gained  successes one after the other \cite{Neal_2018_ECCV,c2ae,gdfr,cgdl}. The Variational Auto-Encoder (VAE) is a typical probabilistic generative model ideal for detecting unknowns, due to its ability in learning low-dimensional representations in latent space not only supporting input reconstruction but also approximating a specified prior distribution. On the other hand, the VAE-based models may be not sufficiently effective for identifying known categories as all feature representations only follow one distribution. So we propose to employ a capsule-based VAE architecture for unknowns detection.

Capsule Networks (CapsNet) \cite{sabour2017dynamic} were proposed by Hinton \etal as an alternative to Convolutional Neural Networks (CNNs). Unlike CNNs’ scalar neurons, capsules ensemble a group of neurons to accept and output vectors. The vector of an activated capsule represents the various properties of a particular object, such as position, size, orientation, texture, etc. In essence, CapsNet can be viewed as an encoder encoding objects by distributed representations, which is exponentially more efficient than encoding them by activating a single neuron in a high-dimensional space. Besides, CapsNet has been successfully used to detect fake images and videos within a task setting similar to open set recognition \cite{fake}. This motivated us to adopt a capsule architecture in combination with VAE for open set recognition. The aim of the proposed model, dubbed VAECapOSR, is depicted in Figure~\ref{fig:VAECapOSR}, i.e., to learn a latent space where instances of features representing a known category are clustered together according to a normal distribution; different known categories are associated to normal distributions with different means, and variances are small enough to obtain well separated clusters; instances in the feature space of unkowns are scattered around the feature space, possibly with no intersection with the clusters representing known categories.

The contribution of this paper can be summarized as follows:
%\begin{enumerate}
%    \item we design a capsule-based variational auto-encoder to get the means and variances of different multivariate Gaussian models for known categories. The model also  embeds a ResNet architecture at the input of the encoder with the aim to learn high-level abstract latent representations for objects in complex backgrounds;
%    \item we develop a novel margin-based loss function to force the posterior distributions of output capsules to approximate different Gaussian models in the latent space;
%    \item we design an ad-hoc  dynamic routing process for CapsNet exploiting a thresholding mechanism to allow capsules in lower layers not to vote any capsule in the higher layers. This novel mechanism enables the clustering process to better adapt to the open set recognition task.
%\end{enumerate}


%%%%%%%%%% Contributions (updated)
\begin{enumerate}
    \item we propose a novel open set recognition framework based on CapsNet architecture and show its advantages and usefulness for learning an efficient representation for known classes;
    \item we integrate CapsNet within VAE architecture and proposed VAECapOSR model. Different from general VAEs that encourage the latent representation to approximate a single prior distribution, our model provide multiple priors, one for each class, and it forces the latent representation to follow the gaussian prior selected by the class of the input sample. %During training, a novel loss function combining the margin loss used in CapsNet and KL-divergence is designed to induce the latent representations to get close to different prior distribution according to their class
    
    
    %Two fully-connected layers are used at the end of CapsNet to project final capsules into a latent embedding space to obtain latent representation for input, where projected latent representations can be redistributed to follow a specific prior distribution.  
    
    
     %A novel loss 
    %\item we propose the integration of CapsNet in the VAE framework for open set recognition. To this end we extended the standard VAE using multiple prior Gaussian distributions for approximating the posterior distribution;
    \item we conduct several experiments, obtaining competitive results, that in some benchmarks outperforms previous state of the art methods by a large margin. 
\end{enumerate}

==> sections/s2_related_work.tex <==
\section{Related Work}
%\subsection{Open Set Recognition}
Open set recognition was defined for the first time by Scheirer \etal \cite{tosr}, who formalized it as a constrained minimization problem. Early works focused on traditional approaches, such as SVM \cite{tosr}, Extreme Value Theory \cite{probinclu, probmod}, sparse representation \cite{srosr} and Nearest Neighbors \cite{nearest}.

Following the success achieved by deep learning in many computer vision tasks, deep networks was first introduced for open set recognition by Bendale \etal \cite{topn}, who proposed an Openmax function by calibrating the Softmax probability of each class with a Weibull distribution model.
Subsequently, to provide explicit probability estimation over unknown classes, \cite{gopenmax} extended Openmax to G-Openmax by introducing a generative adversarial network, in which the generator was able to generate synthetic samples resembling but not belonging to known classes and the discriminator was trained with these samples, in order to learn an explicit representation for unknown classes.
A similar strategy has been also adopted by Neal \etal \cite{Neal_2018_ECCV}, who introduced a data augmentation technique using generative adversarial networks referred as counterfactual image generation.

Yoshihashi \etal \cite{crosr} analyzed and demonstrated the usefulness of deep reconstruction architecture in open set recognition and designed a classification-reconstruction open set recognition framework (CROSR), which combined the supervised learned prediction and unsupervised reconstructive latent representation together to redistribute the probability distribution. Oza et al. \cite{c2ae} first introduced class conditioned VAE to open set recognition and detect unknowns by modelling reconstruction errors with the Extreme Value Theory. Sun et al. \cite{cgdl} argued that one disadvantage of VAE-based architectures for open set recognition was its inadequate discriminative ability for known classes. They employed the probabilistic ladder architecture to develop a conditional Gaussian distribution VAE model (CGDL) for learning conditional distributions for known classes and rejecting unknowns. Zhang et al. introduced a flow-based density estimator into the encoder-decoder architecture to project samples into more representative embedding space. Several experiments showed the promises of the density estimator, but a well-known potential threat was that it may assign higher likelihood to unknown samples. 


==> sections/s3_preliminaries.tex <==
\section{Preliminaries}
In this section, we summarize the background notions needed to introduce our model.

%We start this section introducing the basic notations of open set recognition. Given a labeled training set $\bm{x}\in \mathbb{R}^{N}$ belonging to a set of known classes $\mathcal{K}=\{1, 2,\cdots,N\}$ where $N$ is the number of known classes. The probability of a test sample $\bm{x}$ belongs to a certain known class $C_i$ should be measured by the probability model $P(C_i|\bm{x}, \bm{x} \in \mathcal{K} )$. Besides,the basic architecture of capsule network and the terminology and notation of VAE should be reviewed briefly.
\subsection{Open Set Recognition}
In the open set recognition problem the model has to classify test samples that can belong to classes not seen during training. Considering a classification dataset \mbox{$D = \{(\bm{x}_i, y_i) : 1 \leq i \leq N \}$} with $K$ classes, such that \mbox{$\bm{x}_i \in X$} is an input sample, $y_i \in \mathcal{Y}_c$ is the corresponding category label with $|\mathcal{Y}_c| = K$, the open set problem consists in the classification of test samples among $K + 1$ classes, where the $(K + 1)$-th class is introduced for enabling the recognition of new unseen classes. In the literature, the dataset used for training is called \textit{closed} dataset, meanwhile the one used during evaluation, that contains samples from unseen classes, is called \textit{open} dataset. In order to quantify "how open" is a dataset used for evaluation, following \cite{Neal_2018_ECCV} we define the \textit{openness} measure as $O = 1 - \sqrt{\frac{K}{M}}$ where $K$ and $M$ are  the number of classes observed during training and test, respectively.

\subsection{VAE Formulation}
The VAE is one of the most powerful probabilistic generative models for its theory elegancy, strong framework compatibility and efficient manifold representations. 
The VAEs commonly consist on an encoder that maps the input $\bm{x}$ to a normal gaussian distribution over the latent variable $\bm{z}$, and on a decoder that, given a latent variable $\bm{z}$ tries to reconstruct the input $\bm{x}$.
During training the model is trained my maximizing the variational lower bound, defined as follows:
\begin{equation*}
    \mathcal{L}(\bm{x};\theta,\phi) =  \mathds{E}_{q_\phi (\bm{z}|\bm{x})} \Big[ \log p_\theta (\bm{x}|\bm{z}) \Big] - D_{KL}\Big[ q_\phi (\bm{z}|\bm{x})\|p_\theta(\bm{z}) \Big]
\end{equation*}
where $q_\phi (\bm{z}|\bm{x})$ denotes the posterior of the encoder, and $p_\theta(\bm{z})$ indicates the prior distribution over the latent variable $\bm{z}$. 
The first term in the loss function is the average reconstruction error of the chained encoding-decoding process, while the second term of the loss function is the a regularizer that enforces the approximate posterior distribution $q_\phi(\bm{x}|\bm{z})$ to be close to the prior distribution $p_\theta(\bm{z})$. Original VAE \cite{vae} presumes that $p_\theta(\bm{z})$ is an isotropic multivariate Gaussian $\mathcal{N}(\bm{0}, \bm{I})$ and $q_\phi(\bm{x}|\bm{z})$ is a general multivariate Gaussian $\mathcal{N}(\bm{\mu}, \bm{\sigma^2})$. With these assumptions, the KL-divergence term in the loss function, given a $K$-dimensional $\bm{z}$, can be expressed as,
\begin{equation*}
    D_{KL}\Big[ q_\phi(\bm{z}|\bm{x})\|p_\theta(\bm{z}) \Big] = -\frac{1}{2}\sum_i^K (1+\log (\bm{\sigma}_i^2)-\bm{\mu}_i^2-\bm{\sigma}_i^2).
\end{equation*}
Previous open-set models based on VAE share a similar encoding-decoding framework, and use the latent representation $\bm{z}$ or the reconstruction error between $\bm{x}$ and $\tilde{\bm{x}}$ for outlier detection.

\subsection{CapsNet Formulation}
The conception of capsule was proposed by Hinton et al. \cite{tcap} through encapsulating a group of neurons into the basic units of the network to capture variations of an entity in position, orientation and scale etc. This architecture was further extended by Sabour et al. \cite{sabour2017dynamic} with dynamic routing algorithm and squash function between different capsule layers for preserving the equivariance. For overcoming the insensitivity caused by cosine distance in dynamic routing, Hinton et al. \cite{emrouting} reformulated capsules into matrices and applied EM routing to stack capsule layers, but the expensive computational cost limited its extension to other computer vision tasks. In this paper, we only focus on the dynamic routing capsule network, because it shows better generalization ability with affordble computional cost on natural image datasets, such as SVHN \cite{Netzer2011ReadingDI} and CIFAR10 \cite{Krizhevsky2009LearningML}. CapsNet is a shallow architecture and it is composed by two convolutional layers and two capsule layers. The first convolutional layer with ReLU function converts pixel intensities $\bm{x}$ to primary local feature maps $\vec{\bm{x}}$ that are then used as inputs to primary capsules. Given capsule dimension and channels, the second convolutional operation outputs primary capsules $\mathbf{u}_i$. Each capsule has a set of matrices $\mathbf{W}_{ij}$ multiplied to predict the pose transformation: $\hat{\mathbf{u}}_{j|i}=\mathbf{W}_{ij}\mathbf{u}_i$. Then the classification capsules $\mathbf{v}_j$ can be produced by the weighted sum of the prediction vectors: $\mathbf{v}_j=\sum_ic_{ij}\hat{\mathbf{u}}_{j|i}$, where the coefficients $c_{ij}$ is determined by an dynamic iterative routing process based on the cosine similarity between prediction vectors and classification capsules. For $t$-th iteration, the coefficients are updated by,
\begin{equation*}
    \mathbf{c}^{(t+1)}_{i} = \mathbf{Softmax}(\mathbf{b}^{(t+1)}_i), ~~b^{(t+1)}_{ij} = b^{(t)}_{ij}+\hat{\mathbf{u}}_{j|i}\cdot \mathbf{v}^{(t)}_j.
\end{equation*}
For all layers of capsules, a squash function is used to introduce non-linearity and shrunk the length of capsule vectors into $[0,1]$,
\begin{equation}
    \mathbf{Squash}(\mathbf{v})=\frac{\|\mathbf{v}\|^2}{1+\|\mathbf{v}\|^2}\frac{\mathbf{v}}{\|\mathbf{v}\|}.
\end{equation}



==> sections/s4_proposed_method.tex <==
%%%%%%%%% Proposed Method
\section{Proposed Method}

In this section, we introduce the architecture and the training procedure devised for our proposed model.

%%%%%%%%% Model Architecture
\subsection{Model Architecture}

\begin{figure}[b]
    \centering
    \includegraphics[width=0.5\textwidth]{./plots/openset_model.png}
\caption{Overall scheme of our VAECapOSR model. \label{fig:architecture}}
\end{figure}


%Our model is based on a VAE \cite{vae} with $K$ different gaussian prior distributions, one for each known class. Given an input $\bm{x}$, its representation  $\bm{z}$ produced by the encoder, and the corresponding label $y$, our goal is to structure the features space so to make $\bm{z}$ ``to belong'' to the target gaussian selected by $y$. By doing this, we can make the VAE more discriminative. 

Our proposed model is a CVAE that
From the unsupervised loss in \cite{vae} obtained as the negative lower bound of the log-likelihood of the input data $\bm{x}$, we derive a supervised loss as a function also of the target variable $y$:

\begin{align*}
    \mathcal{L}(\bm{x}, y ;\theta,\phi) =  &D_{KL}\Big[ q_\phi (\bm{z}|\bm{x})\| p_\theta(\bm{z} / y)\Big] \\
    &-\mathds{E}_{q_\phi (\bm{z}|\bm{x})} \Big[ \log p_\theta (\bm{x}|\bm{z}) \Big]
\end{align*}

Minimising such a loss, we force the posterior distribution $q$ to follow the prior distribution $p$ that is conditioned on the class of the input, enforcing the separability of the latent space into class-dependent regions. 

\textbf{Encoder} The encoder $E$ is composed by a features extractor $F$ and a Capsule Network \cite{Sabour2017DynamicRB}. In our work, $F$ is a Residual Network \cite{He2016DeepRL} that is formed by four residual layers. We denote the output of the $l$-th layer as $\bm{x}_l$. After the output of the feature extractor $F$, there is a convolutional layer "CapConv" that reshapes the features %maps 
for the CapsNet, similar to what is done in \cite{Sabour2017DynamicRB}. 

\textbf{CapsNet} The CapsNet produces $K$ mean capsules $\bm{\mu}^{(k)}$ and $K$ variance capsules $\bm{\sigma}^{2(k)}$, each of size $d$. We stack these encoded quantities into blocks of vectors $\bm{\mu} = \left[ \bm{\mu}^{(1)^T} | \bm{\mu}^{(2)^T} | \cdots | \bm{\mu}^{(K)^T} \right]^T$ and \mbox{$\bm{\sigma}^2 = \left[ \bm{\sigma}^{2(1)^T} | \bm{\sigma}^{2(2)^T} | \cdots | \bm{\sigma}^{2(K)^T} \right]^T$}, where $\bm{\mu}, \bm{\sigma}^2 \in \mathbb{R}^{Kd}$, and we denote $\bm{\Sigma} = Diag(\bm{\sigma}^2)$ as the encoded covariance matrix. From now on, we refer to the $j$-th vector block with superscript $(j)$. As introduced in \cite{Sabour2017DynamicRB}, general neurons usually output a scalar value feature for indicating the existence probability of an entity. CapsNets instead, replace the scalar activation with vectorial capsules. When multiple capsules share certain agreement, the capsule with right detection is activated. As a consequence, when the capsule dimension increases, the likelihood of a routing-by-agreement between capsules across a larger cluster with higher dimension decreases significantly. For this reason, we encode the input signal using capsules, and we use CapsNet for open set recognition.  

From now on, we use the superscript $[k]$ to refer to blocks of vectors quantities related to the $k$-th class, and we use the superscript $[k](j)$ to indicate the $j$-th vector block of the quantity corresponding to the $[k]$-th class.

\textbf{Variational Stage} We choose the VAE prior distributions to be $\bm{T}^{[k]} = \mathcal{N} \left( \bm{\mu}^{[k]}, \bm{\mathcal{I}} \right)$ with \mbox{$1 \leq k \leq K$}, with \mbox{$\bm{\mu}^{[k]} = \left[ \bm{\mu}^{[k](1)^T} | \bm{\mu}^{[k](2)^T} | \cdots | \bm{\mu}^{[k](K)^T} \right]^T$} where \mbox{$\bm{\mu}^{[k](j)} = \delta_{k=j} \bm{1}_{d} + \delta_{k \neq j} \bm{0}_{d}$}.
We then sample $\bm{z}$ from $\mathcal{N}(\bm{\mu}, \bm{\Sigma})$, process it through a multi-layer perceptron $MLP(\bm{z}) = relu(BatchNorm(FC(\bm{z})))$ and compute the reconstruction $\bm{\tilde{x}}$ with the decoder $Dec$. 

\textbf{Decoder} We design the decoder network by following a similar architecture of the feature extractor $F$. In order to improve the reconstruction quality, inspired by \cite{Ronneberger2015UNetCN}, we implement lateral connections from the encoder to the decoder, and during training, we randomly dropout the lateral connections for making the decoder less dependent from the internal layers of the encoder. The lateral connections are implemented as \mbox{$LC(\bm{x}_l) = relu(BatchNorm(Conv2d(Dropout(\bm{x}_l))))$.}

The overall forward computation of the model can be summarized as follows:
\begin{align}
    &(\bm{x}_1, \bm{x}_2, \bm{x}_3, \bm{x}_4) = F(\bm{x}), \\
    &(\bm{\mu}, \ \bm{\Sigma}) = CapsNet(CapConv(\bm{x}_4)), \\
    &\bm{z} = \bm{\mu} + \bm{\epsilon} \cdot \sqrt{\bm{\Sigma}}, \ \ \bm{\epsilon} \sim \mathcal{N}(\bm{0}, \bm{\mathcal{I}}), \\
    &\bm{z}_1 = LC_1(\bm{x}), \ \ \bm{z}_2 = LC_2(\bm{x}_1), \\
    &\bm{z}_3 = LC_3(\bm{x}_2), \ \ \bm{z}_4 = LC_4(\bm{x}_3), \\
    &\tilde{\bm{x}} = Dec(MLP(\bm{z}), \bm{z}_1, \bm{z}_2, \bm{z}_3, \bm{z}_4).
\end{align}

%%%%%%%%% Training
\subsection{Training}
We train the model on the closed dataset, and during training for a single input sample $(\bm{x}, y)$ we minimize the negative variational lower bound

\begin{equation}
    \mathcal{L}(\bm{x}, y) = \sum_{k=1}^{K} \mathcal{L}_{KL}^{(k)}(\bm{x}, y) - \beta \mathcal{L}_{rec}(\bm{x}),
\end{equation}
 where 
 
 \begin{align*}
    \mathcal{L}_{KL}^{(k)}(\bm{x}, y) =  
     D_{KL} \left[ \mathcal{N} \big( \bm{\mu}^{(k)}, Diag(\bm{\sigma}^{2(k)}) \big), \bm{T}^{[y](k)} \right] ~~\\
    = \frac{1}{2} \left[ \sum_{i=1}^d (\bm{\sigma}^{2(k)}_i - \log( \bm{\sigma}_i^{2(k)} )  )- d + \| \bm{\mu}^{(k)} - \bm{\mu}^{[y]} \|^2 \right].
 \end{align*}

After the training, we compute for each class $k$ the corresponding class mean and class variance as follows: let $I^{[k]} = \{1 \leq i \leq N \ : \ y_i = k\}$ be the set of indexes selecting all the samples in the $k$-th class, and $N_k$ its cardinality, then the class mean and variance in the latent space are:

\begin{align}
    \bm{\tilde{\mu}}^{[k]} &= \frac{1}{N_k} \sum_{i \in I^{[k]}} \bm{\mu}_i, \\
    \bm{\tilde{\sigma}}^{2[k]} &= \frac{1}{N_k - 1} \sum_{i \in I^{[k]}} (\bm{\mu}_i - \bm{\tilde{\mu}}^{[k]})^2,\\
    \bm{\tilde{\Sigma}}^{[k]} &= Diag(\bm{\tilde{\sigma}}^{2[k]}).
\end{align}


%%%%%%%%% Inference
\subsection{Inference}



\begin{align*}
   \log( P_{in}^{[k]}(\bm{z})) =& 
    -\frac{1}{2}\log( (2\pi)^{Kd} | \bm{\tilde{\Sigma}}^{[k]} |) \\&- \frac{1}{2} (\bm{z} - \bm{\tilde{\mu}}^{[k]})^T ( \bm{\tilde{\Sigma}}^{[k]} )^{-1} (\bm{z} - \bm{\tilde{\mu}}^{[k]}),
\end{align*}


and we use it for classifying the new sample as follows:

\begin{equation*}
  \tilde{y} = \left \{
  \begin{aligned}
    &K + 1, \ \ \text{if}\ \max_{k \in \mathcal{Y}_c} \Big\{ \log( P_{in}^{[k]}(\bm{z})) \Big\} = P^*_{in} < \tau &&\\
    &\argmin_{k \in \mathcal{Y}_c} \Big\{ D_{KL} \big[ \mathcal{N} \left( \bm{\mu}, \bm{\Sigma} \right), \bm{T}^{[k]} \big] \Big\}, \ \ \text{otherwise}. &&
  \end{aligned} \right.
\end{equation*} 

The threshold $\tau$ is selected after training by having $95\%$ of the training samples correctly recognized.

==> sections/s4_proposed_method_old.tex <==
To solve the open set recognition task, our proposed approach comprehends two sub-tasks. As the first stage the model is trained on closed set recognition

In this section, we discuss the two distinctive strengths of CapsNets for open set recognition at first. Then, we present the proposed method in detail including the training phase and the test phase.

\subsection{Motivation}
A typical shortcoming of traditional VAEs for open set recognition is its inadequte ability to provide discriminative representations. Generally, VAEs use a bottleneck architecture to project the input data into a low-dimensional subspace and then reconstruct the input data with the projected intermediate latent representations as well as possible, where the presentations should be forced to follow a specified probability distribution. Therefore, previous open-set works based on VAE assume that all training samples after projection commonly draw the same distribution, thus the well-trained auto-encoders could learn the common reconstructive latent representations from the normal samples and force them approximate a given probability distribution, while anomalous samples could be distinguished because they do not share these common latent representations. However, Xia et al. observe that the above assumption seems to work well only in a specific anomaly setting where the normal samples are drawn from a single class only but anomaly classes can be selected from many other classes \cite{discriRec}. Obviously, such a assumption conflicts with the open-set settings where the normal samples are drawn from multiple classes. The phenomenon is mainly caused by the essential learning mechanism of VAEs, that is to force the posterior distribution of latent representation to approximate one prior distribution. The fact encourages the latent representations of different known classes to get close to the same distribution, thus the discriminative information they contain may be eliminated during this process. A intuitive idea to overcome this shortcoming is to provide a unique prior distribution for each known class. 

CapsNet possesses an intrinsic architecture advantage that is its capability allowing a capsule to use a distributed representation to encode the instantiation parameters of objects appearing in input images. And each target class corresponds to an exclusive capsule indicating its existence. The fact inspires us to devise an architecture allowing different capsules approximate different prior distributions, which would enable CapsNet architecture to learn efficient latent representations for known classes without sacrificing the dircriminative information between them. Logically, these specified prior distributions can be viewed as the centroid of each class which is approximated by the latent representations of corresponding class samples. Besides the dynamic routing between capsule layers, acting as a clustering process, can effectively filter out the contribution of submodules having possibly noisy information and induce those generated representations converge to their corresponding centroids. Therefore, CapsNet architecture is suitable to open set recognition. For inheriting the advantage of VAEs, we force the capsules indicating classes approximate different specified Gaussian distributions. Thus we can assume that a sample is unknown if its latent presentation has a low probability among all prior Gaussian distributions.
\subsection{Architecture}
In the proposed model, the latent representation $\bm{Z}\in \mathbb{R}^{K\times N}$ is the final layer of the encoder. Instead of a linear layer on top of it for label prediction, each known class is assigned with a $K$-dimensional sub-representation $\bm{z}_j$ explicitly indicating its existence, where $\bm{z}_j$ is the $j$-th column of matrix $\bm{Z}$. And the basic framework of the proposed model can be formulated as,
\begin{itemize}
    \item Encoder $\mathcal{F}$: $(\bm{y};\bm{z}_1,\bm{z}_2,\cdots,\bm{z}_N) = \mathcal{F}(\bm{x})$
    \item Decoder $\mathcal{G}$: $\tilde{\bm{x}}=\mathcal{G}(\bm{z}_1,\bm{z}_2,\cdots,\bm{z}_N)$
    \item Unknown Detector $\mathcal{D}$: $P(C_i|\bm{x}, \bm{x} \in \mathcal{K})=\mathcal{D}(\bm{x})$
\end{itemize}
The decoder $\mathcal{G}$ is introduced only being used in training phase to make the latent representation $\bm{z}$ meaningful via reconstruction. $\tilde{\bm{x}}$ is the reconstruction of $\bm{x}$ using $\bm{z}$. To enable the latent representations preserve discriminitive information as much as possible, the output of the decoder $\mathcal{F}$ is formatted as a tuple $(\mathbf{y}, \bm{z})$ where the label $\mathbf{y}$ can be inferred explicitly from the latent representations $\bm{z}$.

\subsection{Encoder}
Unlike the state-of-the-art VAE-based models which heavily rely on \cite{crosr,cgdl} the ladder architecture, the proposed approach is more flexible and can be integrated with various deep neural architectures, such as the dense architecture and the residual architecture (ResNet) \cite{resnet}. Specifically, we preserve the basic architecture of CapsNet and add two linear layers on the top of it to produce a latent representation $\bm{z}_j$ for each classification capsule $\mathbf{v}_j$. Denoting all classification capsules by the matrix $\mathbf{V}=(\mathbf{v}_1,\mathbf{v}_2,\cdots,\mathbf{v}_N)$, we can formulate the operation as,
\begin{align*}
\left(\bm{\mu}_1, \bm{\mu}_2, \cdots, \bm{\mu}_N\right)&=\mathbf{Linear}(\mathbf{V}),\\
(\bm{\sigma}^2_1, \bm{\sigma}^2_2, \cdots, \bm{\sigma}^2_N)&=\mathbf{SoftPlus}(\mathbf{Linear}(\mathbf{V}))\\
\bm{z}_j&=\bm{\mu}_j+\bm{\sigma}_j\odot \epsilon,
\end{align*}
where $\epsilon$ is a disturbance drawn from $\mathcal{N}(0,1)$ and $\odot$ indicates element-wise product, $\bm{\mu}_j$ and $\bm{\sigma}_j$ are the outputs of two linear layers. \textbf{SoftPlus} is a non-linear function $\log (1+\exp (\cdot))$ to ensure all components of its argument are positive. 

To adapt the dynamic process for open-set settings, we devise a mechanism of ``gates" to introduce a ``none-of-the-above'' class for the routing softmaxes. Specifically, for each iteration, we add a learnable bias to the coefficients and activate them with \textbf{ReLU} function,
\begin{align*}
b_{ij}&=\mathbf{v}_j\cdot \hat{\mathbf{u}}_{i|j}, \\
\mathbf{c}_j&=\mathbf{Softmax}_i(b_{ij}), \\
\mathbf{c}_j&=\mathbf{ReLU}(\mathbf{c}_j+\mathbf{bias})
\end{align*}
Without such an operation, when all cosine similarities $b_{ij}$ approximate zero, the softmax function have to distribute equal weights to all high-level capsules, ie. all components of the coefficients $\mathbf{c}_j$ would approximate $1/N$ unreasonably. The gates can learn a bias for the voting weights, whose values less than the bias will be compressed to zero. It is important for open set recognition that this operation allows ``none-of-the-above" routing results.

\subsection{Decoder}
In previous works \cite{crosr,c2ae,cgdl}, the decoder plays an important role in unknown detection because the reconstruction loss error is modeled as a detecting indicator. Therefore, it is necessary to design a decoder with similar architecture complexity as the encoder to ensure that the reconstructed images are effective and usable as well as possible. Besides, to avoid some important features and factors vanishing in the bottleneck architecture of the decoder, intermediate representations from different layers of the encoder are embedded into the corresponding-level layers of the decoder via various interaction methods.

In our approach, we have weakened the importance of the detector in unknown detection and only use it to prevent the encoder generating over-degraded latent representations. The encoder tends to produce highly similar outputs for each class during optimization, which may cause the difficulty to fit them with a Gaussion distribution. Thus we adopt a simple decoder with 3 fully connected layers and 3 transposed convolutional layers.

\subsection{Loss Function}
The objective of loss function design is to induce the network to learn efficient latent representations facilitating open set recognition. In general, we hope the representations belonging to the same class are as close to each other as possible but the representations belonging to different classes are far from each other, that is to potentially compress the overlap domain between known classes and unknown classes in the latent subspace. Ideally, the representations of samples from known classes should follow or approximate a prior distribution, in which novelty can be detected easily if the probability is lower than a given threshold. The KL-divergence used in most VAEs' loss function is a good candidate to encourage the approximate posterior $q_\phi$ of the encoder to be close to a prior $q_\theta$. Thus our intuitive idea is to utilize KL-divergence to regulate the output of the proposed network. We expect the linear maps of activated top-level capsules are close to $\mathcal{N}(0,1)$ but others are not. In practice, the $j$-th capsule is encouraged to follow $\mathcal{N}(0,1)$ if and only if the input image is of class $j$, other $N-1$ capsules are enforced to approximate $\mathcal{N}(1,1)$. Thus the margin loss for $j$-th capsule is design as,
\begin{equation*}
\mathcal{L}_j=\bm{y}_j\cdot D_{KL}(\bm{z}_j, \mathcal{N}(0,1))+\lambda(1-\bm{y}_j)\cdot D_{KL}(\bm{z}_j, \mathcal{N}(1,1)).
\end{equation*}
where $\bm{y}_j=1$ if and only if the input is belongs to class $j$. The $\lambda$ down-weighting of the loss for absent classes stops the initial learning from enforce all activity vectors approximating $\mathcal{N}(0,1)$. Thus the total loss including the reconstruction loss $\mathcal{L}_\mathrm{recon}$ can be expressed by,
\begin{equation*}
\mathcal{L}_\mathrm{total}=\sum_{j=1}^N\mathcal{L}_j+\beta \mathcal{L}_\mathrm{recon},
\end{equation*}
where the hyper-parameter $\beta$ is empirically taken as 0.0005 for balancing the mean squared error and the KL-divergence of all capsules.

During the training phase, the loss function forces the conditional posterior $q_\phi ((\bm{z}_1,\bm{z}_2,\cdots,\bm{z}_N)|\bm{x}, j)$ to approximate different multivariate Gaussian distribution,
\begin{align*}
    \bm{z}_1 &\sim \mathcal{N}(\bm{1}, \bm{1}),\\
    \bm{z}_2 &\sim \mathcal{N}(\bm{1}, \bm{1}),\\
    &\cdots \\
    \bm{z}_j &\sim \mathcal{N}(\bm{0}, \bm{1}),\\
    &\cdots \\
    \bm{z}_N &\sim \mathcal{N}(\bm{1}, \bm{1}),
\end{align*}
if and only if the input belongs to the $j$-th class. For closed-set label prediction, unlike original CapsNet using the length of classification capsules to indicate class-belongingness, the proposed model determines the prediction label by
\begin{equation*}
    \mathbf{Softmax}\left(\frac{1}{D_{KL}(\bm{z}_j, \mathcal{N}(\bm{0},\bm{1}))+\epsilon} \right),
\end{equation*}
where $\epsilon$ is a positive real number which prevents the denominator from becoming zero.
\subsection{Unknown Detector}
The variational capsules make a very strong representational assumption that the latent representation of all correctly classified training samples in $j$-th class approximate a multivariate Gaussian distribution $\Phi (\bm{z}_1^\mathrm{T},\bm{z}_1^\mathrm{T},\cdots, \bm{z}_N^\mathrm{T})$, and we model the distribution by $\mathcal{N}(\bm{u}_j,\bm{m}_j)$, where $\bm{u}_j$ and $\bm{m}_j$ are the mean and the variance of vector-form latent representations $(\bm{z}_1^\mathrm{T},\bm{z}_1^\mathrm{T},\cdots, \bm{z}_N^\mathrm{T})$ separately. The sample predicted to be class $j$ if the probability $\Phi (\bm{z}_1^\mathrm{T},\bm{z}_1^\mathrm{T},\cdots, \bm{z}_N^\mathrm{T})$ exceeds a given threshold $\tau_j$ for class $j$.

It is noting that the selection of a reasonable threshold for each class affects significantly the performance of the unknown detector, we need to find a balance between keeping the training examples while rejecting unknown examples. Given a set of training samples belonging to class $j$, we sort their probability ${\Phi_j}$ according to ascending rule and select a threshold by ensuring 95\% training data to be recognized as knowns. Besides, in case of the fail detection of the Gaussian model caused by abnormal value, the $L^2$ norm between the latent representation and the class centroid is used to determine unknowns, whose threshold $\tau_\alpha$ is still based on ensuring 95\% training data to be recognized as knowns. The details of the test procedure is described in Algo. 1.
\begin{algorithm}
\caption{Test procedure.}
\label{alg}
\begin{algorithmic}
 \Require
      Well-trained modules $\mathcal{F}$, $\mathcal{G}$\;
\Require
    compute the latent representation $(\bm{z}^\mathrm{T}_1, \bm{z}^\mathrm{T}_2,\cdots, \bm{z}^\mathrm{T}_N)_k$ for each correctly classified training sample $\bm{x}_k$\;
\State For each class $j$, compute the representation $(\bm{z}^\mathrm{T}_1, \bm{z}^\mathrm{T}_2,\cdots, \bm{z}^\mathrm{T}_N)_k$ for each correctly classified training sample $\bm{x}_k$,\\
      
\For{ $j=1,2,\cdots,N$}
\State$\bm{u}_j=mean_k((\bm{z}^\mathrm{T}_1, \bm{z}^\mathrm{T}_2,\cdots, \bm{z}^\mathrm{T}_N)_k)$,
\State$\bm{m}_j=mean_k((\bm{z}^\mathrm{T}_1, \bm{z}^\mathrm{T}_2,\cdots, \bm{z}^\mathrm{T}_N)_k)$,
\State $\Phi_j(\bm{z}^\mathrm{T}_1, \bm{z}^\mathrm{T}_2,\cdots, \bm{z}^\mathrm{T}_N)=\mathcal{N}(\bm{u}_j,\bm{m}_j)$.
\EndFor
\State for a test sample $\bm{x}$, $(\bm{y}_\mathrm{pred};\bm{z}_1,\bm{z}_2,\cdots,\bm{z}_N)=\mathcal{F}(\bm{x})$,\
\If{$\forall j\in \{1,2,\cdots, N\}, \Phi_j(\cdot)<\tau_j$ or $L^2$-norm $> \tau_\alpha$}
\State predict $x$ as unknown
\Else
\State predict $x$ as known with label $\bm{y}_\mathrm{pred}$
\EndIf
\end{algorithmic}
\end{algorithm}

==> sections/s5_experimental_results.tex <==
%%%%%%%%%% Experimental Results
\section{Experimental Results}

In this section, we present the experimental settings used to evaluate the performance of the proposed approach, and we compare our model with respect to state of the art methods for open set recognition.
\subsection{Datasets}

We evaluate open set classification performance on several benchmarks, such as MNIST~\cite{lecun-mnisthandwrittendigit-2010}, SVHN~\cite{Netzer2011ReadingDI}, CIFAR10~\cite{Krizhevsky2009LearningML}, CIFAR+10, CIFAR+50 and TinyImageNet~\cite{Le2015TinyIV} datasets and, for a fair comparison, we reuse the same splits provided by~\cite{Neal_2018_ECCV}.

\textbf{MNIST, SVHN, CIFAR10} All three datasets contain ten categories. MNIST contains monochrome images with hand-written digits, and it has $60000$ $28\times28$ gray images for training and $10000$ for testing. SVHN contains street view house numbers, consisting of ten digit classes each with between $9981$ and $11379$ $32\times32$ color images. To validate our method on non-digital images, we use the CIFAR10 dataset, which has $50000$ $32\times32$ natural color images for training and $10000$ for testing. Following the protocol in~\cite{Neal_2018_ECCV}, for the unknown detection task, each dataset is randomly partitioned into $6$ known classes and $4$ unknown classes. In these setting, the openness score is fixed to $22.54\%$.

\textbf{CIFAR+10, CIFAR+50} To test the our model in a setting of higher openness values, we perform CIFAR+$Q$ experiments using CIFAR10 and CIFAR100~\cite{Krizhevsky2009LearningML}. $4$ known classes are sampled from CIFAR10 and $Q$ unknown classes are drawn randomly from the more diverse and larger CIFAR100 dataset. Openness scores of CIFAR+10 and CIFAR+50 are $46.54\%$ and $72.78\%$, respectively.

\textbf{TinyImageNet} For TinyImagenet dataset, which is subset of the ImageNet that contains $200$ classes, we randomly sampled $20$ classes as known and the remaining classes as unknown. In this setting, the openness score is $68.37\%$.


%%%%%%%%%% Metrics
\subsection{Metrics}

Open set classification performance can be characterized by F-score and AUROC (Area Under ROC Curve)~\cite{Geng2020RecentAI}. 
F-score is used for measuring the in-distribution classification performance, while AUROC is commonly reported by both open set recognition and out-of-distribution detection literature. AUROC provides a calibration free measure and characterizes the performance for a given score by varying the discrimination threshold. For our experiments, we use macro averaged F1-score on the open set recognition task, and the AUROC for the unknown detection task.
For both metrics, higher values are better.


%%%%%%%%%% Results
\subsection{Results}

%%%%%%%%%% Unknown detection
Following \cite{cgdl} we conducted two different experiments in which our model has to solve the \textit{unknown detection} task and the \textit{open set recognition} task.
In the \textit{unknown detection} problem the model is trained on a subset of the dataset using $K$ classes, and the evaluation is done by measuring the model capability on detecting unknown classes, not seen during training. The evaluation is performed by considering the binary recognition task of the known vs unknown classes, and in this experiment we adopt the AUROC measure previously discussed. The results, shown in Table~\ref{tab:auc}, are averaged over five different random splits of known and unknown classes, provided by~\cite{Neal_2018_ECCV}. In the MNIST and SVHN datasets we outperform all previous methods while in the CIFAR10, CIFAR+10, CIFAR+50 and TinyImageNet dataset we note a drop in the performances. We investigated the protocols adopted by the other models \footnote{We have run the released code by CGDL without achieving their results. We provide the our obtained results in the supplementary material.} that achieves better performances on CIFAR10, CIFAR+10, CIFAR+50 and TinyImageNet, but they don't mention whether they use the same data splits as done in~\cite{Neal_2018_ECCV}, the one we used.

\begin{table*}
    \centering
    \begin{tabular}{l|c|c|c|c|c|c} \hline
    Method     &   MNIST & SVHN & CIFAR10 & CIFAR+10 & CIFAR+50 & TinyImageNet \\
    \hline
    Softmax~\cite{cgdl}    & 0.978 & 0.886 & 0.677 & 0.816 & 0.805 & 0.577 \\
    Openmax~\cite{topn}    & 0.981 & 0.894 & 0.695 & 0.817 & 0.796 & 0.576 \\
    G-Openmax~\cite{gopenmax}  & 0.984 & 0.896 & 0.675 & 0.827 & 0.819 & 0.580 \\
    OSRCI~\cite{Neal_2018_ECCV}      & 0.988 $\scriptstyle{\pm 0.004}$ & 0.91 $\scriptstyle{\pm 0.01}$ & 0.699 $\scriptstyle{\pm 0.038}$ & 0.838 & 0.827 & 0.586 \\
    CROSR~\cite{crosr}    & 0.991 $\scriptstyle{\pm 0.004}$ &  0.899 $\scriptstyle{\pm  0.018}$ & - & - & - & 0.589 \\
    C2AE~\cite{c2ae}       & 0.989 & 0.922 & 0.895 & 0.955 & 0.937 & 0.748 \\
    CGDL~\cite{cgdl}       & 0.994 $\scriptstyle{\pm 0.002}$ & 0.935 $\scriptstyle{\pm 0.003}$ & 0.903 $\scriptstyle{\pm 0.009}$ & 0.959 $\scriptstyle{\pm 0.006}$ & 0.950 $\scriptstyle{\pm 0.006}$ & 0.762 $\scriptstyle{\pm 0.005}$ \\ 
    OpenHybrid~\cite{hybrid}  & \underline{0.995} & \underline{0.947} & \textbf{\underline{0.950}} & \textbf{\underline{0.962}} & \textbf{\underline{0.955}} & \textbf{\underline{0.793}} \\
    \hline
    VAECapOSR (ours)       & \textbf{0.997} $\scriptstyle{\pm 0.002}$ & \textbf{0.953} $\scriptstyle{\pm 0.002}$ &  0.823 $\pm$ $\scriptstyle{\pm 0.012}$ &  0.868 $\scriptstyle{\pm 0.008}$ & 0.829 $\scriptstyle{\pm 0.009}$ &  0.706  $\scriptstyle{\pm 0.004}$ \\ \hline
    \end{tabular}
    \caption{AUROC scores on the detection of known and unknown samples. Results are averaged among 5 different splits of known and unknown classes partitions.}
    \label{tab:auc}
\end{table*}


%%%%%%%%%% Open set recognition

In the \textit{open set recognition} problem, as previously mentioned, the model is trained on the closed dataset that contains $K$ classes, and it is evaluated on the open dataset considering $K + 1$ classes. In this experimental setting, we evaluate the model using the macro F1-score on the $K + 1$ classes. In the first experiment for open set recognition, we train on all the classes of the MNIST dataset and we then evaluate the performances by including new datasets in the open set. Similar to~\cite{crosr} we used Omniglot, MNIST-Noise, and Noise that are datasets of gray-scale images. Each of this dataset contains $10000$ test images, the same as MNIST, and an example of how they appear is reported in Fig.~\ref{fig:mnist_outliers}. The Omniglot dataset contains hand-written characters from the alphabets of many languages, while the Noise dataset has images synthesized by randomly sampling each pixel value independently from a uniform distribution on $[0, 1]$. MNIST-Noise is also a synthesized set, constructed by superimposing MNIST’s test images on Noise. The results of the open set recognition on these datasets are shown in Table~\ref{mnist}. On each dataset, we outperform state-of-the-art results by a large margin. On Omniglot, we improve the F1-score by $+0.121$, in the MNIST-Noise by $+0.095$, and in the Noise by $+0.123$. We also report the t-SNE~\cite{Maaten2008VisualizingDU} visualization of the latent space of the open test set in Figure~\ref{fig:t-sne}. 

\begin{figure}[ht]
    \centering
    \begin{tabular}{m{0.14\textwidth} m{0.3\textwidth}}
         MNIST & \includegraphics[width=0.25\textwidth]{./plots/mnist.png} \\
         Omniglot & \includegraphics[width=0.25\textwidth]{./plots/omniglot.png} \\
         MNIST-Noise & \includegraphics[width=0.25\textwidth]{./plots/mnist_noise.png} \\
         Noise & \includegraphics[width=0.25\textwidth]{./plots/noise.png} \\
    \end{tabular}
    \caption{Samples of MNIST, Omniglot, MNIST-Noise, and Noise datasets.}
    \label{fig:mnist_outliers}
\end{figure}

\begin{table}[ht]
    \centering
    \begin{tabular}{l|l|l|l}\hline
     Method  &  Omniglot & MNIST-noise & Noise  \\ \hline
     Softmax~\cite{cgdl} &  0.595    & 0.801       & 0.829  \\
     Openmax~\cite{gopenmax} &  0.780    & 0.816       & 0.826  \\
     CROSR~\cite{crosr}   &  0.793    & 0.827       & 0.826  \\
     CGDL~\cite{cgdl}    &  \underline{0.850}    & \underline{0.887}       & \underline{0.859}  \\ \hline
     VAECapOSR (ours)    &  \textbf{0.971}   & \textbf{0.982}      & \textbf{0.982} \\ \hline
    \end{tabular}
    \caption{Results for the open set recognition on the MNIST dataset. We reported the macro-averaged F1-score in $11$ classes ($10$ from the test partition of the MNIST, and $1$ from the test of another dataset).}
    \label{mnist}
\end{table}

\begin{figure*}[ht]
    \centering
    \begin{tabular}{c c c c}
    
        \begin{subfigure}[b]{0.27\textwidth}
            \centering
            \caption{Omniglot Open Set}
            \includegraphics[width=\textwidth]{./plots/tsne_omniglot_v2.png}
            
            \label{fig:t-sne_omniglot}
         \end{subfigure} &

         \begin{subfigure}[b]{0.27\textwidth}
            \centering
            \caption{MNIST-Noise Open Set}
            \includegraphics[width=\textwidth]{./plots/tsne_mnist_noise_v2.png}
            
            \label{fig:t-sne_mnist_noiet}
         \end{subfigure} &

         \begin{subfigure}[b]{0.27\textwidth}
            \centering
            \caption{Noise Open Set}
            \includegraphics[width=\textwidth]{./plots/tsne_noise_v2.png}
            
            \label{fig:t-sne_noise}
         \end{subfigure} &

        \begin{subfigure}[t]{0.11\textwidth}
            \centering
            \includegraphics[width=\textwidth]{./plots/tsne_legend_v5.png}
         \end{subfigure} \\
         

    \end{tabular}
    \caption{t-SNE visualizations of the test open set MNIST features computed by the encoder. The test open set includes the test samples from MNIST and the test samples from the unknown datasets. Fot all the figures, the unknown samples coming from the unknown datasets are marked with black triangles.}
    \label{fig:t-sne}
\end{figure*}


In the second experiment of open set recognition, following the same protocol as in~\cite{Neal_2018_ECCV}, all samples of the $10$ classes in CIFAR10 dataset are considered as known data, and samples from ImageNet and LSUN are selected as unknown samples. For having the same image size respect to known samples, we resize or crop the unknown samples, obtaining the following datasets: ImageNet-crop, ImageNet-resize, LSUN-crop, and LSUN-resize. For each dataset, we consider all their $10000$ test samples as the unknown samples in the open set. The performance of the method is evaluated using the macro-averaged F1-scores in the $11$ classes ($10$ known classes and 1 unknown), and the results are shown in Table~\ref{tab:cifar}. We can see that our method shows competitive F1-score on ImageNet-resize, and outperform all previous state of the art models on ImageNet-crop, LSUN-crop, and LSUN-resize. 


\begin{table*}
    \centering
    \begin{adjustbox}{width=\linewidth,center}
	\setlength{\tabcolsep}{12pt}
    \begin{tabular}{l|l|l|l|l}\hline
    Method             & ImageNet-crop & ImageNet-resize & LSUN-crop & LSUN-resize \\
    \hline
    Softmax~\cite{cgdl}            & 0.639         &0.653  &0.642  &0.647 \\
    Openmax~\cite{topn}            & 0.660         &0.684  &0.657  &0.668 \\
    LadderNet+Softmax~\cite{crosr}  & 0.640         &0.646  &0.644  &0.647 \\
    LadderNet+Openmax~\cite{crosr}  & 0.653         &0.670  &0.652  &0.659 \\
    DHRNet+Softmax~\cite{crosr}     & 0.645         &0.649  &0.650  &0.649 \\
    DHRNet+Openmax~\cite{crosr}     & 0.655         &0.675  &0.656  &0.664 \\
    CROSR~\cite{crosr}             & 0.721         &0.735  &0.720  &0.749 \\
    C2AE~\cite{c2ae}               & 0.837         &0.826  &0.783  &0.801 \\
    CGDL~\cite{cgdl}               & \underline{0.840}         & \underline{0.832}  & \underline{0.806} & \underline{0.812} \\
    \hline
    VAECapOSR (ours) & \textbf{0.857} & \textbf{0.834}  & \textbf{0.868} & \textbf{0.882} \\
    \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Results for the open set recognition on CIFAR-10 with various outliers added to the test set as unknowns. We evaluate the model using macro-averaged F1-scores in $11$ classes ($10$ from the the test of the CIFAR10, and $1$ from various test datasets.)}
    \label{tab:cifar}
\end{table*}


%%%%%%%%%% Ablation on model architecture
\textbf{Ablation study on the model architecture.} In order to verify the contribution of each part of our model, we perform ablation on the relevance of the major model's components: the \textit{CapsNet}, the feature extractor \textit{F} and the dynamic routing algorithm in the \textit{CapsNet}. We investigate also the impact of the dynamic routing procedure on open set recognition, in order to understand its importance. We consider four different variations of our model architecture: \textit{CapsNet} that don't use the ResNet feature extractor, but just a single convolutional layer for massaging the input, and uses dynamic routing. \textit{ResNet20+CapsNet} that includes the residual feature extractor before the \textit{CapsNet} and don't uses dynamic routing, \textit{ResNet20+FC} where a fully connected layer replaces the \textit{CapsNet}, and \textit{ResNet20+CapsNet+DR} that implements dynamic routing in the \textit{CapsNet}. For all \textit{CapsNets} that don't implement the dynamic routing, we process each capsule with a fully connected layer. For the ablation we consider the SVHN dataset as the closed dataset, and we consider unknown samples form the CIFAR100 for the open dataset. We then consider different number of unknown classes of CIFAR100, leading to different openness values $O$. The ablation analysis is reported in Table~\ref{tab:abalation}. We can see that the residual network used as a feature extractor in the encoder helps, specially when the openness $O$ of the open set increases. This fact highlight the importance of having already pre-processed features for the \textit{CapsNet} on unknown detection when openness increases. Another emerging fact is the importance of having the \textit{CapsNet} respect of having a \textit{FC} layer: as the openness increases, the AUROC improvement increases until $+0.344$. This result suggests that capsules are more capable on detecting unknown samples respect to standard artificial neurons. Finally, we see that dynamic routing achieves better performances respect to not using it, and this fact highlights the importance of using capsules with dynamic routing.

\begin{table*}[!t]

    \centering
    \begin{adjustbox}{width=\linewidth,center}
	\setlength{\tabcolsep}{5pt}
    \begin{tabular}{l c c c c c c}\hline
    \multicolumn{7}{ c }{AUROC @ different Openness Values $O$}\\
    \hline
    \hline
     VAECapOSR Variation   &$O=0\%$     &$O=15.98\%$   &$O=24.41\%$   &$O=30.72\%$   &$O=35.67\%$   &$O=39.69\%$ \\
     \hline
     \hline
     \multicolumn{7}{ c }{Importance a Feature Extractor before CapsNet}\\
     \hline
     CapsNet    &0.971   &0.753	  &0.760	 &0.767	    &0.774	   &0.781   \\
     ResNet20+CapsNet     &\textbf{0.981}   &\textbf{0.948}     &\textbf{0.949}     &\textbf{0.949}     &\textbf{0.949}     &\textbf{0.950}   \\
     \hline
     Improv.     &+0.020   &+0.195	  &+0.189	 &+0.182	    &+0.175	   &+0.169   \\
     \hline
     \hline
     \multicolumn{7}{ c }{CapsNet Importance}\\
     \hline
     ResNet20+FC            &0.975   &0.581	  &0.586	 &0.595	    &0.601	   &0.606   \\
     ResNet20+CapsNet     &\textbf{0.981}   &\textbf{0.948}     &\textbf{0.949}     &\textbf{0.949}     &\textbf{0.949}     &\textbf{0.950}   \\
     \hline
     Improv.     &+0.006   &+0.367	  &+0.363	 &+0.354	    &+0.348	   &+0.344   \\
     \hline
     \hline
     \multicolumn{7}{ c }{Dynamic Routing Importance}\\
     \hline
     ResNet20+CapsNet     &0.981   &0.948     &0.949     &0.949     &0.949     &0.950   \\
     ResNet20+CapsNet+DR  &\textbf{0.982}    &\textbf{0.952}       &\textbf{0.953}   &\textbf{0.954}   &\textbf{0.954}    &\textbf{0.955}\\ 
     \hline
     Improv.     &+0.001   &+0.004	  &+0.004	 &+0.005	    &+0.005	   &+0.005   \\
     \hline
    \end{tabular}
    \end{adjustbox}
    \caption{Ablation study of the architecture of our model. Here we reported the performances of our model for the unknown detection task on SVHN dataset with various outliers from CIFAR100. The performance is evaluated by AUROC with different openness values.}
    \label{tab:abalation}

\end{table*}

==> sections/s6_conclusion.tex <==
\section{Conclusion}
In this paper we introduce VAECapOSR, a model for open set recognition based on VAE that produces latent representations using CapsNets. We extended the standard framework of VAEs using multiple gaussian prior distributions rather than just one for all known classes in the closed dataset. Experimental results show the high performances of the proposed model on unknown detection and open set recognition tasks, even improving by a large margin the state of the art results on MNIST.
